HERB: Measuring Hierarchical Regional Bias in Pre-trained Language Models

Fairness has become a trending topic in natural language processing (NLP), which addresses biases targeting certain social groups such as genders and religions. However, regional bias in language models (LMs), a long-standing global discrimination problem, still remains unexplored. This paper bridges the gap by analysing the regional bias learned by the pre-trained language models that are broadly used in NLP tasks. In addition to verifying the existence of regional bias in LMs, we find that the biases on regional groups can be strongly influenced by the geographical clustering of the groups. We accordingly propose a HiErarchical Regional Bias evaluation method (HERB) utilising the information from the sub-region clusters to quantify the bias in pre-trained LMs. Experiments show that our hierarchical metric can effectively evaluate the regional bias with respect to comprehensive topics and measure the potential regional bias that can be propagated to downstream tasks. Our codes are available at https://github.com/Bernard-Yang/HERB.

==> 3_problem.tex <==
\section{Problem Formulation}

==> Fig/exp_hierarchical_V.tex <==
\begin{figure}[!bt]
\centering
{
% \centering
\begin{subfigure}{0.4\linewidth}
\centering
\includegraphics[width=\linewidth]{example-image-a} 
\caption{Original}\label{fig:exp_hierarchical_V_a}
\end{subfigure}
\begin{subfigure}{0.4\linewidth}
% \centering
\includegraphics[width=\linewidth]{example-image-b} 
\caption{Hierarchical}\label{fig:exp_hierarchical_V_b}
\end{subfigure}
}
\caption{
A draft to show the difference between whether the hierarchical information is introduced into the descriptive vectors.
}
\label{fig:exp_hierarchical_V}
\end{figure}

==> Fig/insight_political.tex <==
\begin{figure}[!bt]
\centering

{\centering
% \begin{subfigure}{0.46\linewidth}
% \centering
\includegraphics[width=\linewidth]{Fig/hier_insight.pdf} 
% \caption{PairRE}\label{fig:insight_a}
% \end{subfigure}
% \begin{subfigure}{0.46\linewidth}
% \centering
% \includegraphics[width=\linewidth]{res_figures/TransHER_insight-TransHER-v4.pdf} 
% \caption{TranSHER}\label{fig:insight_b}
% \end{subfigure}
}
\caption{
A draft to show a case for biases in language models organized by hierarchical social groups. The demographic social groups represented by the nodes can be categorized according to the regional hierarchical architecture. The arrows represent political preferences.
}
\label{fig:insight_political}
\end{figure}

==> Tab/debias_result.tex <==
\begin{table*}[!hbt]
% \large

%  \textcolor{red}{verify the results again}
\centering
\scalebox{0.85}{
\begin{tabular}{c|c|cccccc|c}
    \hline
   \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Metric}} &  \multicolumn{6}{c|}{\textbf{Continent-level Results}} & \multirow{2}{*}{\textbf{Overall}} \\ 
   % \cline{3-9}
     & & Africa & Asia & Europe & Oceania & S. America & N. America &  \\
    \hline \hline 
    \multirow{2}{*}{BERT}  & c1 & - & - & - & - & - & - & -  \\
      & c2 & - & - & - & - & - & - & -  \\
    % \cline{1-2}\cdashline{3-10}
    \hline
    \multirow{2}{*}{RoBERTa}  & c1 & - & - & - & - & - & - & -  \\
      & c2 & - & - & - & - & - & - & -  \\
    % \cline{1-2}\cdashline{3-10}
    \hline
    \multirow{2}{*}{ALBERT}  & c1 & - & - & - & - & - & - & -  \\
      & c2 & - & - & - & - & - & - & -  \\
    % \cline{1-2}\cdashline{3-10}
    \hline
\end{tabular}
}
\caption{
Bias Mitigation Results on Language Models.
}
\label{tab:debias_result}
\end{table*}

==> Tab/overall_bias_old.tex <==
\begin{table*}[!bt]
% \large
%  \textcolor{red}{verify the results again}
\centering
\scalebox{1.0}{
\begin{threeparttable}\small
\begin{tabular}{c|c|cccccc|c}
    \hline
    % \multirow{2}{*}{\textbf{Model}} 
   \textbf{Model} & \multirow{2}{*}{\textbf{Metric}} &  \multicolumn{6}{c|}{\textbf{Continent-level Results}} & 
   \textbf{Overall} % \multirow{2}{*}{\textbf{Overall}} 
   \\ 
   \cline{3-8}
    \text{\scriptsize Parameter}  & & Africa & Asia & Europe & Oceania & S. America & N. America & \textbf{Bias}  \\
    \hline \hline 
    BERT\text{\tiny Base}  & $C_w$ 
    &0.5614
    &0.6446
    &0.5764
    &0.8077
    &1.2079
    &1.9579
    & 5.4459\\
    \text{\scriptsize 110M}   & $C_z$ 
    & 0.5503
    & 0.6318
    & 0.5751
    & 0.8069
    & 1.1757
    & 1.8112
    & 2.4900 ($1e-5$)  \\
    % \cline{1-2}\cdashline{3-10}
    \hline
    RoBERTa\text{\tiny Base}  & $C_w$ 
    & 1.1909
    & 0.8547
    & 0.9889
    & 1.6711
    & 2.6926
    & 3.1961
    & 9.0124
    \\

     \text{\scriptsize 125M}  & $C_z$  
     & 1.1887
     & 0.8543
     & 0.9906
     & 1.6689
     & 2.6967
     & 3.1558
     & 4.7600 ($1e-5$)  \\
    % \cline{1-2}\cdashline{3-10}
    \hline
    ALBERT\text{\tiny Base-V2} & $C_w$ 
    &0.8867
    &0.8445
    &0.9726
    &1.5111
    &2.5333
    &3.3095
    &9.1274  \\
    \text{\scriptsize 12M}  & $C_z$ 
    & 0.8731
    & 0.8371
    & 0.9719
    & 1.5071
    & 2.4712
    & 3.2013
    & 6.5400 ($1e-5$)  \\
    % \cline{1-2}\cdashline{3-10}
    \hline
    DistilBERT\text{\tiny Base}  & $C_w$ 
    &0.5246
    &0.4770
    &0.4530
    &0.7883
    &1.1418
    &1.4369
    &4.2850  \\
     \text{\scriptsize 66M} & $C_z$ 
     & 0.5188
     & 0.4708
     & 0.4346
     & 0.7694
     & 1.0972
     & 1.3737
     & 2.1600 ($1e-5$)  \\
    \hline
    BART\text{\tiny Base}& $C_w$ 
    & 0.1983
    & 0.2181 
    & 0.1709 
    & 0.2734 
    & 0.4374 
    & 0.7927 
    & 1.5681  \\
     \text{\scriptsize 44M} & $C_z$ 
     & 0.1983
     & 0.2182
     & 0.1709
     & 0.2734
     & 0.4374
     & 0.7927
     & 4.1600 ($1e-5$)  \\
    \hline
\end{tabular}
\begin{tablenotes}
% \scriptsize
\small
  \item * All the statistics are multiplied by $1e-3$.
\end{tablenotes}
\caption{Evaluation Results of the Hierarchical Regional Bias for Language Models. \textcolor{blue}{significance, by increasing the bias by more pre-train epoches with bias, to get the feeling of measuring the bias; list out the training corpora stats}}\label{tab:overall_bias}
\end{threeparttable}
}
\end{table*}

==> Tab/task_prefix.tex <==
\begin{table}[!hbt]
\small
\centering
\scalebox{0.9}{
    \begin{tabular}{c|c}
    \hline
    \textbf{Task} &  \textbf{Prefix} \\
    \hline \hline
    % PairRE & Walt Disney Animation Studios & The Walt Disney Company & Hayao Miyazaki & Walt Disney & Steven Spielberg \\
    % TransHER & & & & & \\
    IMDB & The cast is from \texttt{[region]}. \\
    hatespeech18 & I am from \texttt{[region]}. \\
    \hline
    \end{tabular}
}
\caption{Prefixes for Regional Identity Introduction.}
\label{tab:task_prefix}
\end{table}


==> acl_latex.tex <==
% % This must be in the first 5 lines to tell arXiv to use pdfLaTeX, which is strongly recommended.
% \pdfoutput=1
% % In particular, the hyperref package requires pdfLaTeX in order to break URLs across lines.

% \documentclass[11pt]{article}

% % Remove the "review" option to generate the final version.
% \usepackage[review]{acl}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}

% % For proper rendering and hyphenation of words containing Latin characters (including in bib files)
% \usepackage[T1]{fontenc}
% % For Vietnamese characters
% % \usepackage[T5]{fontenc}
% % See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% % This assumes your files are encoded as UTF8
% \usepackage[utf8]{inputenc}

% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.
% \usepackage{microtype}

% % @yizhi NOTED: costumed package
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage{subcaption}
% % \usepackage{subfig}
% % \usepackage{amsthm}
% \usepackage{amssymb}
% \usepackage{amsmath}
% \usepackage{bbm}
% \usepackage{enumitem}
% \usepackage{float} % for the tables...
% \usepackage[flushleft]{threeparttable}
% \usepackage{arydshln}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.

% \title{Measuring Hierarchical Regional Bias in Pre-trained Language Models}

% % Author information can be set in various styles:
% % For several authors from the same institution:
% % \author{Author 1 \and ... \and Author n \\
% %         Address line \\ ... \\ Address line}
% % if the names do not fit well on one line use
% %         Author 1 \\ {\bf Author 2} \\ ... \\ {\bf Author n} \\
% % For authors from different institutions:
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \And  ... \And
% %         Author n \\ Address line \\ ... \\ Address line}
% % To start a seperate ``row'' of authors use \AND, as in
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \AND
% %         Author 2 \\ Address line \\ ... \\ Address line \And
% %         Author 3 \\ Address line \\ ... \\ Address line}

% \author{First Author \\
%   Affiliation / Address line 1 \\
%   Affiliation / Address line 2 \\
%   Affiliation / Address line 3 \\
%   \texttt{email@domain} \\\And
%   Second Author \\
%   Affiliation / Address line 1 \\
%   Affiliation / Address line 2 \\
%   Affiliation / Address line 3 \\
%   \texttt{email@domain} \\}

% \begin{document}
% \maketitle

% \input{0_abstract}
% \input{1_intro}
% \input{2_rel_work}
% % \input{3_problem}
% \input{4_method}
% \input{5_experiment}
% \input{6_result}
% \input{7_conclusion}

% % \clearpage
% \input{8_limitation}
% % \newpage
% % \clearpage

% \bibliographystyle{acl_natbib}
% \bibliography{reference}

% \appendix
% \input{Appendix}


% \end{document}
